The Query Complexity of Certification

We study the problem of {\sl certification}: given queries to a function $f : \{0,1\}^n \to \{0,1\}$ with certificate complexity $\le k$ and an input $x^\star$, output a size-$k$ certificate for $f$'s value on $x^\star$. This abstractly models a central problem in explainable machine learning, where we think of $f$ as a blackbox model that we seek to explain the predictions of. For monotone functions, a classic local search algorithm of Angluin accomplishes this task with $n$ queries, which we show is optimal for local search algorithms. Our main result is a new algorithm for certifying monotone functions with $O(k^8 \log n)$ queries, which comes close to matching the information-theoretic lower bound of $\Omega(k \log n)$. The design and analysis of our algorithm are based on a new connection to threshold phenomena in monotone functions. We further prove exponential-in-$k$ lower bounds when $f$ is non-monotone, and when $f$ is monotone but the algorithm is only given random examples of $f$. These lower bounds show that assumptions on the structure of $f$ and query access to it are both necessary for the polynomial dependence on $k$ that we achieve.

==> FORC_abstract.tex <==
We study the problem of {\sl certification}: given queries to a function $f : \zo^n \to \zo$ with certificate complexity $\le k$ and an input $x^\star$, output a size-$k$ certificate for $f$'s value on~$x^\star$. 

For monotone functions, a classic local search algorithm of Angluin accomplishes the certification task with~$n$ queries, which we show is optimal for local search algorithms.  Our main result is a new algorithm for certifying monotone functions with $O(k^8 \log n)$ queries, which comes close to matching the information-theoretic lower bound of $\Omega(k \log n)$.  The design and analysis of our algorithm are based on a new connection to threshold phenomena in monotone functions.

We further prove exponential-in-$k$ lower bounds when $f$ is non-monotone, and when $f$ is monotone but the algorithm is only given random examples of $f$.  These lower bounds show that assumptions on the structure of $f$ and query access to it are both necessary for the polynomial dependence on $k$ that we achieve.

==> findanycert.tex <==
\section{Finding an arbitrary certificate}

In this section we show how to find an \textit{arbitrary} certificate of a monotone function in $O(k^7\log n)$ queries where $k$ is the certificate complexity of the function. We first state the algorithm below then show each step can be implemented in a query efficient manner and with high probability of success. In particular, we'll give a $O(k^7\log k\log(n))$ query upper bound and then we'll show how a simple modification of the algorithm can obtain a $O(k^7\log n)$ upper bound. 

\begin{algorithm}
\begin{algorithmic}[1]
\Require A monotone function $f:\{0,1\}^n\to \{0,1\}$.
\State Initialize $\pi\leftarrow \varnothing$
\While{$f$ is nonconstant}
\State Estimate $p^*$, the critical probability of $f$
\State Estimate $\Inf_{i,p^*}[f]$ for all $i$
\State Add coordinate $i$ to $\pi$ where $\Inf_{i,p^*}[f]$ is the largest influence estimate
\State $f\leftarrow f_{x_i=b}$ where $b=0$ if $p^*\ge 1/2$ and $1$ otherwise
\EndWhile
\State \Return the certificate $\pi$
\end{algorithmic}
\caption{Finding a certificate of a monotone function}
\label{alg:arbitrary_certificate}
\end{algorithm}

When the critical probability $p^*$ reaches $1$ or $0$ the function must be constant and hence the restricted coordinates form a certificate. As such, our progress measure for \Cref{alg:arbitrary_certificate} is the critical probability $p^*$. One of the main ideas is that if $\E_{p^*}[f]$ is close to $1/2$ then the maximum $p^*$-influence of $f$ is at least $\Omega(1/k^2)$ where $k$ is the certificate compleixty of $f$. Moreover we can show that restricting $f$ according to the index with the largest influence ensures that the critical probability of the restricted function $f_b$ is at least $\Omega(1/k^3)$ greater than or less than the critical probability of $f$. Thus we get a $O(k^3)$ upper bound on the number of coordinates restricted before $f$ is constant and hence an $O(k^3)$ upper bound on the size of the certificate returned. 


\begin{theorem}
\label{theorem:find_cert_algo_correctness}
\Cref{alg:arbitrary_certificate} whp\footnote{Throughout this work, whp will mean with probability $1-1/\poly(n)$.} returns a certificate of size $O(k^3)$ and makes $O(k^7\log k\log n)$ total queries to $f$. 
\end{theorem}

Before proving \Cref{theorem:find_cert_algo_correctness} we establish a few claims. A key ingredient in our analysis is the Russo-Margulis lemma which was originally proved independently by Margulis in \cite{Mar74} and Russo in \cite{Rus78} in the context of graph theory and percolation theory. O'Donnell proves a Fourier analytic version of the lemma in \cite{ODBook}. We give a self-contained proof of the lemma in \Cref{appendix:rm_lemma}.

\begin{lemma}[Russo-Margulis Lemma]
    \label{lemma:russo_margulis}
    Let $f$ be a monotone function, then 
    $$
    \frac{d}{dp}\E_p[f]=\Inf_{p}[f].
    $$
\end{lemma}

An important corollary of this lemma allows us to relate the certificate complexity of $f$ to the $p$-biased expectation of $f$. 

\begin{corollary}
    \label{corollary:tangent_certificate}
    Let $f:\{0,1\}^n\to\{0,1\}$ be a monotone function with $C(f)\le k$, then for all $p_0\neq p_1$ we have
    $$
    \frac{\E_{p_1}[f]-\E_{p_0}[f]}{p_1-p_0}\le k.
    $$
\end{corollary}

\begin{proof}
    By the mean value theorem, the slope of the tangent line $(\E_{p_1}[f]-\E_{p_0}[f])/(p_1-p_0)$ is the derivative of $\E_p[f]$ at some point in between $p_1$ and $p_0$. Hence combining with \Cref{lemma:russo_margulis} there is some $\hat p$ satisfying
    $$
    \frac{\E_{p_1}[f]-\E_{p_0}[f]}{p_1-p_0}=\left.\frac{d}{dp}\E_p[f]\right\rvert_{p=\hat p}=\Inf_{i,\hat p}[f].
    $$
    By \Cref{claim:basic_props}, $\Inf_{\hat p}[f]=\E_{\hat p}[\Sens_f(x)]$. It follows $\Inf_{\hat p}[f]\le C(f)$ because the sensitivity of an input lower bounds its certificate complexity. \Cref{fig:proof_slope_bound} illustrates this idea.
\end{proof}


% \pgfplotsset{width=\linewidth,compat=newest}
\begin{figure}
    \begin{center}
    % \resizebox{\linewidth}{!}{
    \begin{tikzpicture}
    \begin{axis}[
            scale only axis,
            width=0.7\linewidth,
            xtick={0,1},
            % ytick={0,1},
            xticklabels={0,1},
            ytick={0,0.5,1},
            yticklabels={0,$\frac{1}{2}$,1},
            xmin=0, xmax=1,
            ymin=0, ymax=1,
            xlabel = {$p$},
            % x label style = {at={(1,0)}},
            ylabel = {},
            y label style = {rotate=-90},
            % yticklabel style = {text width=-0.8\linewidth},
            axis lines=left,
            clip=false,
            legend pos=north west,
        ]
        % line y=1/2
        \addplot[gray, dashed, forget plot] coordinates {(0,0.5) (1,0.5)};
        
        % p-expectation of f
        \addplot[color=blue,smooth,thick,-,domain=0:0.4368, forget plot] {3.35985*x^2.3};
        \addplot[color=blue,smooth,thick,-,domain=0.4368:1] {2.7987*(x-1)^(3)+1};
        % \addlegendimage{line width=0.3mm,color=blue}
        \addlegendentry{$\E_p[f]$}
        
        % p-expectation of f_0
        \addplot[color=red,smooth,thick,-,domain=0:0.5, forget plot] {10*x^5.5};
        \addplot[color=red,smooth,thick,-,domain=0.5:1] {-3.116*(x-1)^2+1};
        \addlegendentry{$\E_p[f_0]$}
        
        % derivative point and tangent line
        \node[draw,circle,fill=black,inner sep=1.5pt] (derivative) at (0.5,0.221) {};
        \addplot[mark=none, black] coordinates {(0.45,0.0996) (0.55,0.342)};
        
        % tangent line slope derivative 
        \draw[color=black] (0.55,0.3) node[align=center] (label) [below right] {\small $\begin{aligned}
            \frac{\E_{p(f_0)}[f_0]-\E_{p(f)}[f_0]}{p(f_0)-p(f)}&=\left.\frac{d\E_p[f]}{dp}\right\rvert_{p=\hat p}\\
            &=\Inf_{\hat p}[f]\\
            &\le C(f)
        \end{aligned}$};
        
        % curved arrow
        \draw[<-] (derivative) edge [out=0, in=180]  (label);
        
        % point E_{p(f)}[f0]
        \node[draw,circle,fill=black,inner sep=1.5pt] (epf0) at (0.4368,0.1051) {};
       
        % labels for p(f) and p(f0)
        \draw[] (0.4368,0.5) node [above,fill=white!30] {$p(f)$};
        \draw[color=black] (0.5994,0.5) node [above,fill=white] {$p(f_0)$};
        
        % point p(f)
        \node[draw,circle,fill=black,inner sep=1.5pt] (p) at (0.4368,0.5) {};
        
        % point p(f0)
        \node[draw,circle,fill=black,inner sep=1.5pt,] (p0) at (0.5994,0.5) {};
       
        % arrow for p(f0)-p(f) distance
        % \draw [decorate,decoration={brace,raise=2pt}] (p) -- (p0) node [black,pos=0.5,yshift=0.5cm] { $\Omega(1/k^3)$};
        \draw [<->] (p) -- (p0) node[midway,below,fill=white!30] {$\Omega(1/k^3)$};
        
        % arrow for Epf[f0] to 1/2
        \draw[<->] (p) -- (epf0) node[midway,left,fill=white!30] {$p(f)\Inf_{i,p(f)}[f]$};
        
        % tangent line connecting p0 and p1
        \draw[black, thick, dotted] (epf0) -- (p0);
        
    \end{axis}
\end{tikzpicture}
% }
\end{center}
\caption{Illustration of the proof of \Cref{theorem:find_cert_algo_correctness} using \Cref{corollary:tangent_certificate}. The top curve illustrates $\E_p[f]$ as a function of $p$ and the lower curve illustrates $\E_p[f_0]$ where $f_0$ is obtained from $f$ by restricting one of its coordinates to $0$. The points $p(f)$ and $p(f_0)$ mark the critical probabilities of $f$ and $f_0$ respectively.}
\label{fig:proof_slope_bound}
\end{figure}
The Russo-Margulis Lemma helps us understand how much the critical probability of $f$ changes as we restrict the coordinates of $f$. Specifically with this corollary, we can show that even an approximation of the critical probability of $f$ can ensure good progress. 

\begin{claim}
    \label{claim:p_progress}
    Let $f$ have certificate complexity $k$ and let $p\in[0,1]$ satisfy $\E_p[f]\in [1/2-\varepsilon,1/2+\varepsilon]$ and let $i$ satisfy $\Inf_{i,p}[f]\ge\tau$. Then for $b\in\{0,1\}$ and the restriction $f_{x_i=b}$, for any $p_b$ satisfying $\E_{p_b}[f_b]\in [1/2-\varepsilon,1/2+\varepsilon]$ we have
    $$
    \frac{p\tau-2\varepsilon}{k}\le p_0-p
    $$
    and
    $$
    \frac{(1-p)\tau-2\varepsilon}{k}\le p-p_1
    $$
\end{claim}
    
\begin{proof}
Let $p_b$ be as in the statement of the claim. Using \Cref{claim:basic_props} part (6) we have
$$
\E_p[f_0]=\E_p[f]-p\Inf_{i,p}[f].
$$
Thus, by \Cref{corollary:tangent_certificate} we can write
\begin{align*}
    k&=\frac{\E_{p_0}[f_0]-\E_p[f_0]}{p_0-p}\\
    &=\frac{\E_{p_0}[f_0]-\E_p[f]+p\Inf_{i,p}[f]}{p_0-p}\\
    &\ge \frac{-2\varepsilon+p\tau}{p_0-p}
\end{align*}
where we use the assumption that $\E_p[f],\E_{p_b}[f_b]\in [1/2-\varepsilon,1/2+\varepsilon]$ and so $\E_{p_0}[f_0]-\E_p[f]\ge -2\varepsilon$. An analogous computation for $f_1$ using 
$$
\E_p[f_1]=\E_p[f]+(1-p)\Inf_{i,p}[f]
$$
shows that
$$
k\ge \frac{-2\varepsilon+(1-p)\tau}{p-p_1}.
$$
\end{proof}


To estimate the critical probability as required in the statement of \Cref{claim:p_progress}, we need the following claim. 

\begin{claim}
    \label{claim:expectation_bounds}
    Let $f$ have certificate complexity $k$ and critical probability $p^*$. Then $p\in [p^*-\varepsilon,p^*+\varepsilon]$ implies $\E_p[f]\in [1/2-k\varepsilon,1/2+k\varepsilon]$.
\end{claim}
    
\begin{proof}
We write
$$
k\ge \frac{\E_{p^*}[f]-\E_{{p^*}-\varepsilon}[f]}{{p^*}-({p^*}-\varepsilon)}=\frac{1/2-\E_{{p^*}-\varepsilon}[f]}{\varepsilon}
$$
and hence by monotonicity $1/2-k\varepsilon\le\E_{{p^*}-\varepsilon}[f]\le \E_{p}[f]$ for all $p\ge {p^*}-\varepsilon$. An anlogous computation shows that $1/2+k\varepsilon\ge \E_{{p^*}+\varepsilon}[f]\le \E_p[f]$ for all $p\le {p^*}+\varepsilon$. 
\end{proof}

And finally the lower bound the influence as required in the statement of \Cref{claim:p_progress} we use the OSSS inequality \cite{OSSS05}. This inequality states that $\max_i\widetilde{\Inf}_{i,p}[f]\ge \Var_p[f]/D(f)$ where $D(f)$ is the decision tree depth of $f$ and $\widetilde{\Inf}_{i,p}[f]$ is \textit{rerandomized} influence. That is
$$\widetilde{\Inf}_{i,p}[f]=2\underset{\bx\sim\{0,1\}_p^n}{\Pr}[f(\bx)\neq f(\bx^{(i)})]$$
where $x^{(i)}$ is the string $x$ with the $i$th bit rerandomized according to $\{0,1\}_p$. Since we have $\widetilde{\Inf}_{i,p}[f]=4p(1-p)\Inf_{i,p}[f]\le \Inf_{i,p}[f]$ the OSSS inequality also holds for our definition of influence. For our analysis, we also apply the bound $D(f)\le C(f)^2$ to obtain OSSS in terms of certificate complexity.

\begin{fact}[OSSS inequality]
\label{claim:OSSS}
Let $f:\{0,1\}^n\to\{0,1\}$ satisfy $C(f)\le k$ then
$$
\max_i \Inf_{i,p}[f]\ge \frac{\Var_p[f]}{k^2}
$$
\end{fact}

Influence and critical probability can both be estimated with high accuracy using random sampling. The following claim specifies more precisely how many samples are needed to achieve a high degree of confidence.

\begin{claim}
\label{claim:random_sample}
Fix some $f:\{0,1\}^n\to\{0,1\}$ and $p\in[0,1]$ and let $\Phi_f(p)=\E_p[f]$.
Then for any $\varepsilon,\delta>0$, $\Phi_f$ can be estimated with accuracy $\pm \varepsilon$ and with confidence $1-\delta$ using $O(1/\varepsilon^2\log(1/\delta))$ many random samples from $\{0,1\}_p^n$. That is if we let $\bX$ be the random variable denoting an estimate of $P_f$ using $O(1/\varepsilon^2\log(1/\delta))$ random samples then
$$
\Pr\left[\bX\in [\Phi_f(p)-\varepsilon,\Phi_f(p)+\varepsilon] \right]\ge 1-\delta.
$$
\end{claim}
\begin{proof}
Suppose we take $k$ random samples of $\{0,1\}_p^n$ and write $\bX_i$ for the $i$th indicator of the $i$th sample -- that is $\bX_i$ is $1$ if $f(x)=1$ and $0$ otherwise. Then $\Pr[\bX_i=1]=\Pr_p[f(\bx)=1]=\Phi_f(p)$ and hence $\sum_{i=1}^k \bX_i\sim \text{Bin}(k,\Phi_f(p))$. It follows then from a Chernoff bound for random sampling that the estimate $\bX=\sum_{i=1}^k \bX_i/k$ satisfies
$$
\Pr\left[\bX\in [\Phi_f(p)-\varepsilon,\Phi_f(p)+\varepsilon] \right]\ge 1-\delta
$$
for any $\varepsilon,\delta>0$ and $k\ge O(1/\varepsilon^2\log(1/\delta))$.
\end{proof}

With these claims we can now prove the correctness of the algorithm.

\begin{proof}[Proof of \Cref{theorem:find_cert_algo_correctness}]

Our proof proceeds by first showing that we can estimate the critical probability of $f$ and the influences accurately enough to ensure quick progress towards termination. Then we show that we can estimate these quantities to the specified accuracy with high probability using few queries.

\noindent
\textbf{Accurately estimating the critical probability and influences}. Our measure of progress is the critical probability of $f$. At a high level we can show that if the critical probability is accurate to within an additive factor of $O(1/k^3)$ and each influence to within a factor of $O(1/k^2)$ then the critical probability of $f_b$ is guaranteed to increase or decrease by $O(1/k^3)$. Since the function is constant when the critical probability is $0$ or $1$ we know that the algorithm must terminate after $O(k^3)$ steps. 

To be more specific, let $f$ be a nonconstant function obtained at some point in the algorithm with $C(f)\le k$. Write $\overline{p}$ for an estimate of $p^*$, the critical probability of $f$, using random samples and likewise let $\overline{\Inf}_{i,\overline{p}}[f]$ be an estimate for the $i$th influence. Now suppose
\begin{enumerate}
    \item $\E_{\overline{p}}[f]\in [1/2-1/128k^2,1/2+1/128k^2]$
    \item $\overline{\Inf}_{i,\overline{p}}[f]\in[\Inf_{i,\overline{p}}[f]-1/16k^2,\Inf_{i,\overline{p}}[f]+1/16k^2]$.
\end{enumerate}
Then we show if $\overline{p}\ge 1/2$ we have 
$$
\overline{p}+\frac{1}{64k^3}\le \overline{p_0}
$$
and conversely if $\overline{p}< 1/2$ we have
$$
\overline{p}-\frac{1}{64k^3}\ge \overline{p_1}
$$
where $\overline{p_b}$ is the respective estimate for $f_b$ (which is also estimated to the same accuracy as $p^*$). Specifically by \Cref{claim:expectation_bounds} we have $\E_{\overline{p}}[f]\in [1/2-1/128k^2,1/2+1/128k^2]$. Recalling $f$ is monotone and $\Var_p[f]=\E_p[f](1-\E_p[f])$ we have $\Var_{\overline{p}}[f]\ge (1/2-1/128k^2)(1/2+1/128k^2)\ge 1/8$. By \Cref{claim:OSSS} we can then bound $\max_i\Inf_{i,\overline{p}}[f]\ge 1/8k^2$ which ensures that 
$$
\max_i \overline{\Inf}_{i,\overline{p}}[f]\ge \max_i\Inf_{i,\overline{p}}[f]-\frac{1}{16k^2}\ge \frac{1}{16k^2}. 
$$
Finally applying \Cref{claim:p_progress} with $\tau=1/16k^2$ and $\varepsilon=1/128k^2$ we get that 
$$
\overline{p_0}-\overline{p}\ge \frac{\overline{p}(1/16k^2)-1/64k^2}{k}=\frac{1}{16k^3}\left(\overline{p}-\frac{1}{4}\right) 
$$
and 
$$
\overline{p}-\overline{p_1}\ge \frac{1}{16k^3}\left((1-\overline{p})-\frac{1}{4}\right).
$$
In the final step of the algorithm $f$ is restricted to $x_i=0$ if $\overline{p}\ge 1/2$ in which case we have $\overline{p_0}-\overline{p}\ge 1/64k^3$ by the above and otherwise $x_i$ is restricted to $1$ and $\overline{p}<1/2$ which ensures that $\overline{p}-\overline{p_1}\ge 1/64k^3$. Note importantly that if $\overline{p}\ge 1/2$ the next estimate will also be greater than $1/2$ and so on, ensuring that the final certificate will be a $0$-certificate. Otherwise, the estimate remains less than $1/2$ throughout the algorithms execution and the resulting certificate will be a $1$-certificate. In either case, one step of the main loop makes at least $\Omega(1/k^3)$ progress towards termination and so the loop iterates $O(k^3)$ times. Hence, the final certificate has at most $O(k^3)$ coordinates since each iteration of the loop adds one coordinate. 

\noindent
\textbf{Query efficiency}. We show that with error probability $1/\poly(n)$ we can estimate $\overline{p}$ using $O(k^4\log k\log n)$ queries to $f$ and we can estimate $\overline{\Inf}_{i,\overline{p}}[f]$ using $O(k^4\log n)$ queries to $f$. The algorithm makes these estimates at most $O(k^3)$ times giving the upper bound $O(k^7\log k \log n)$. 

To estimate $\overline{p}$ we can split the unit interval $[0,1]$ into $O(k^3)$ subintervals each of length $O(1/k^3)$ and perform binary search to find the interval which contains the critical probability. By \Cref{claim:expectation_bounds} we know the interval containing the critical probability will satisfy $\E_{p}[f]\in [1/2-1/128k^2,1/2+1/128k^2]$ for all $p$ in that interval, and by \Cref{claim:random_sample} we can use random samples to estimate $\E_p[f]$ with accuracy $\pm 1/128k^2$ and confidence $1-\delta$ using $O(k^4\log(1/\delta))$ samples. We perform this estimation $O(\log k)$ times during the binary search, and this binary search takes place once for each of the $O(k^3)$ iterations of the algorithm so the total number of queries is $O(k^7\log k\log(1/\delta))$. We can choose $\delta=1/\poly(n)$ to be small enough so that by a union bound the probability of making any incorrect estimate during the course of the algorithm is at most $1/\poly(n)$. Then the overall number of queries is $O(k^7\log k\log n)$. 

To estimate influences we write
$$
\Inf_{i,p}[f]=\Pr_p[f_1(x)\neq f_0(x)]=\E_p[f_1-f_0]
$$
using \Cref{claim:basic_props}. Thus, we again use \Cref{claim:random_sample} to estimate $\Inf_{i,p}[f]$ to accuracy $\varepsilon=1/16k^2$ and confidence $\delta$ using $O(k^4\log(1/\delta))$ random samples. We choose $\delta=1/\poly(n)$ small enough so that the probability any estimate is incorrect is at most $1/\poly(n)$ by a union bound. The total number of random samples for one iteration of the loop is then $O(k^4\log n)$ making the total number of queries $O(k^7\log n)$ to estimate influences.
\end{proof}

\subsection{Reducing the query complexity via fewer critical probability estimates}

We can reduce the query complexity of \Cref{alg:arbitrary_certificate} by a $\log k$ factor if we instead estimate the critical probability of $f$ once at the beginning of the algorithm then deterministically update it by the error term we calculated as $1/128k^3$ in the proof above. At a high level, the idea is that the analysis for \Cref{theorem:find_cert_algo_correctness} shows that restricting $f$ by an influential coordinate should shift it's critical probability by at least $\Omega(1/k^3)$. Hence, in the worst case, the algorithm makes the smallest amount of progress, $1/k^3$, in each step. We can thus manually shift our critical probability estimate after each iteration by the minimal amount of progress we expect instead of using additional queries to $f$ to determine the new critical probability. This modification is formalized in the claim below.


\begin{claim}
    \label{claim:p_progress_deterministic}
    Fix an error term $0<\varepsilon\le 1/(64k^3)$ and let our initial estimate $\overline{p}_0$ of the critical probability of $f$ satisfy $\overline{p}_0\in [p_0-\varepsilon,p_0+\varepsilon]$. Assume that $\overline{p}_0\ge 1/2$. Let $\overline{p}_t=t\varepsilon+\overline{p}_0$ be the estimate of the critical probability used at the $t$ step of \Cref{alg:arbitrary_certificate}. Suppose furthermore that each influence estimate satisfies $\overline{\Inf}_{i,\overline{p}_t}[f]\in [\Inf_{i,\overline{p}_t}[f]-2k\varepsilon,\Inf_{i,\overline{p}_t}[f]+2k\varepsilon]$. Then for all $t$, we have $p_t\ge p_0+t\varepsilon$ where $p_t$ and $p_0$ are the true critical probabilies of $f$ at the $t$th and $0$th steps of the algorithm.
\end{claim}


\begin{proof}[Proof sketch]
    The proof is by induction on $t$. If $t=0$, then the statement is immediate. Otherwise assume that $p_t-p_0\ge t\varepsilon$. Then we show $p_{t+1}-p_0\ge (t+1)\varepsilon$. If $p_t\ge (t+1)\varepsilon+p_0$ then the statement follows since $p_{t+1}\ge p_t$. Otherwise, assume that $p_t\in [p_0+t\varepsilon,p_0+(t+1)\varepsilon]$. Since $\overline{p}_t=\overline{p}_0+t\varepsilon$ and $\overline{p}_0\in [p_0-\varepsilon,p_0+\varepsilon]$ we have $\overline{p}_t\in [p_0+(t-1)\varepsilon, p_0+(t+1)\varepsilon]\subseteq [p_t-2\varepsilon,p_t+\varepsilon].$ We can then use \Cref{claim:expectation_bounds} as in the proof of \Cref{theorem:find_cert_algo_correctness} to deduce that $\Var_{\overline{p_t}}[f_t]\ge 1/8$. Similarly, we can show that 
    $$
    \max_i \overline{\Inf}_{i,\overline{p}_t}[f_t]\ge \frac{1}{8k^2}-2k\varepsilon.
    $$
    Finally applying \Cref{claim:p_progress} we can combine the above to show
    \begin{align*}
        k&\ge \frac{\E_{p_{t+1}}[f_{t+1}] -\E_{\overline{p}_t}[f_{t+1}]}{p_{t+1}-\overline{p}_t}\\
        &=\frac{1}{p_{t+1}-\overline{p}_t}\cdot\paren{\frac{1}{16k^2}-2k\varepsilon}
    \end{align*}
    which shows 
    $$
    p_{t+1}-p_0-(t-1)\varepsilon\ge p_{t+1}-\overline{p}_t\ge 2\varepsilon
    $$
    after using the assumption that $\varepsilon\le 1/(64k^3)$. 
\end{proof}

Note that the assumption in \Cref{claim:p_progress_deterministic} that $\overline{p}_0\ge 1/2$ is without loss of generality since the argument for the case $\overline{p}_0<1/2$ is symmetric (in this case we'd simply have $\overline{p}_t=\overline{p}_0-t\varepsilon$). 

As a corollary, we can modify \Cref{alg:arbitrary_certificate} slightly to reduce the overall query complexity by a $\log k$ factor.

\begin{corollary}
    \label{corollary:arbitrary_alg_upper_bound}
    Given a monotone function $f:\{0,1\}^n\to\{0,1\}$ with $C(f)\le k$, there is an algorithm which whp returns a certificate of size $O(k^3)$ and makes $O(k^7\log n)$ queries to $f$. 
\end{corollary}
\begin{proof}
    Simply modify \Cref{alg:arbitrary_certificate} to only estimate the critical probability of $f$ at the start and then increment/decrement it by $\varepsilon=1/16k^3$ after each iteration. Then the algorithm terminates after at most $O(k^3)$ iterations of the main loop by \Cref{claim:p_progress_deterministic}.  Also, the same query analysis from the proof of \Cref{theorem:find_cert_algo_correctness} applies although we only estimate the critical probability once which makes $O(k^4\log k\log n)$ queries. Then one iteration of the loop requires $O(k^4\log n)$ queries and hence the algorithm overall makes $O(k^7\log n)$ queries. 
\end{proof}



==> shapley.tex <==
\section{Lower bounds on Shapley variance and Shapley values}
In this section, we show that $\sv[f]$ is $\Omega(1/d)$ when $f$ is given by a decision tree of depth $d$.  A key ingredient in establishing a lower bound for the Shapley variance is a relation between the $p$-biased expectation of $f$ and the $p$-biased influence. In particular, the derivative with respect to $p$ of $\E_p[f]$ is \textit{exactly} the $p$-biased influence. This result is known as the Russo-Margulis Lemma.
\begin{lemma}[Russo-Margulis Lemma]
\label{lem:russomargulis}
Let $f$ be a monotone function then
$$
\frac{d}{dp}\E_p[f]=\Inf_p[f].
$$
\end{lemma}

With this we can prove the main theorem. 

\begin{theorem}
\label{theorem:sv_lower}
Let $f$ be a nonconstant monotone function with a decision tree of depth $d$, then
$$
\sv[f]\ge \Omega\paren{\frac{1}{d}}
$$
and more specifically $\sv[f]\ge 1/64d$. 
\end{theorem}
\begin{proof}
We first observe that, using Claim \ref{claim:basic_props} that
$$
\Inf_p[f]=\underset{x\sim\{0,1\}_p^n}{\E}[\Sens_f(x)]\le d
$$
because for every $x$, $\Sens_f(x)\le d$. It follows by Lemma \ref{lem:russomargulis} that $d/dp\E_p[f]\le d$. This shows that $d/dp\Var_p[f]\le d$ because $\Var_p[f]\le \E_p[f]$. 

Since $\E_p[f]$ is monotone increasing on $(0,1)$ (as $f$ is nonconstant and $\inf_p[f]> 0$) we have that $\Var_p[f]=\E_p[f](1-\E_p[f])$ is monotone increasing in any interval for which $\E_p[f]\in (0,1/2)$. In particular, $\Var_p[f]$ attains a maximum at $1/4$. Let $p^*$ denote the unique point for which $\Var_{p^*}[f]=1/4$. Fix some $\eps\in (0,1/4)$ and let $p_1<p^*$ be such that $\Var_{p_1}[f]=1/4-\eps$ so that $\Var_p[f]\ge 1/4-\eps$ for all $p\in [p_1,p^*]$. Then by the mean value theorem we know that there is some point for which the derivative of $\Var_p[f]$ is equal to
$$
\frac{\Var_{p^*}[f]-\Var_{p_1}[f]}{p^*-p_1}=\frac{1/4-(1/4-\eps)}{p^*-p_1}=\frac{\eps}{p^*-p_1}
$$
which shows that
$$
\frac{\eps}{p^*-p_1}\le d
$$
by our observation that the derivative of $\Var_p[f]$ is bounded by $d$ and hence $p^*-p_1\ge \eps/d$. It follows that
\begin{align*}
    \underset{p\sim[0,1]}{\E}\left[\Var_p[f]\right]&\ge \underset{p\sim[p_1,p^*]}{\E}[\Var_p[f]]\\
    &\ge \underset{p\sim[p_1,p^*]}{\E}[1/4-\eps]\\
    &=(1/4-\eps)(p^*-p_1)\\
    &\ge (1/4-\eps)\frac{\eps}{d}\\
    &=\frac{1}{d}\paren{\frac{\eps}{4}-\eps^2}.
\end{align*}
Choosing $\eps=1/8$ maximizes this lower bound and shows that
$$
\sv[f]=\underset{p\sim[0,1]}{\E}\left[\Var_p[f]\right]\ge \frac{1}{64d}.
$$
as desired.
\end{proof}


\subsection{An OSSS inequality for Shapley values}

The authors in \cite{OSSS05} give an upper bound of the form
$$
\Var[f]\le\sum_{i=1}^n\delta_i(T)\Inf_i[f]
$$
where $\delta_i(T)$ is the probability $x_i$ is queried in a given decision tree $T$ for $f$. The inequality holds when the variance, probability, and influence are taken over any product distribution. Informally, we call an inequality of this form an \textit{OSSS inequality} (after the authors' names in \cite{OSSS05}). Our goal is to prove an OSSS inequality for Shapley variance:
$$
\sv[f]\le\sum_{i=1}^n\delta_i(T)\shap_i[f].
$$
We first state the precise result from \cite{OSSS05} that we use in our proof. We write $\Inf_{i,p}^{\text{OSSS}}[f]$ to denote the influence of the $i$th variable of $f$ under the $p$-biased distribution using in \cite{OSSS05}. They define this quantity as
$$
\Inf_{i,p}^{\hspace{0.1em}\text{OSSS}}[f]=2\underset{x\sim\{0,1\}_p^n}{\Pr}[f(x)\neq f(x^{(i)})]
$$
where $x^{(i)}$ is the string $x$ with the $i$th bit rerandomized according $\{0,1\}_p$. We can show that their definition of influence is upper bounded by our definition. If we let
$$
T=\{x\in\{0,1\}^n\mid f(x)\neq f(x^{\oplus i})\text{ and } x_i=1\}
$$
then
\begin{align*}
    \Inf_{i,p}^{\hspace{0.1em}\text{OSSS}}[f]&=2\sum_{x\in T}p\Pr_p[x\mid x_i=1](1-p)+(1-p)\Pr_p[x^{\oplus i}\mid x^{\oplus i}_i=0]p\\
    &=2\sum_{x\in T}2p(1-p)\Pr_p[x\mid x_i=1]\\
    &=4p(1-p)\sum_{x\in T}\Pr_p[x\mid x_i=1]\\
    &=4p(1-p)\sum_{x\in T}p\Pr_p[x\mid x_i=1]+(1-p)\Pr_p[x^{\oplus i}\mid x^{\oplus i}_i=0]\\
    &=4p(1-p)\Inf_{i,p}[f]\\
    &\le \Inf_{i,p}[f]
\end{align*}
where we use the fact that $\Pr_p[x\mid x_i=1]=\Pr_p[x^{\oplus i}\mid x^{\oplus i}_i=0]$ as both probabilities only depend on the non-$i$th bits of $x$. 

Before establishing an OSSS inequality for Shapley variance, we relate the Shapley values of $f$ to its $p$-biased influence.



\begin{theorem}
\label{theorem:osss}
Let $f$ be a Boolean function with decision tree $T$ and let $\delta_i^p(T)=\Pr_p[{T\text{ queries }x_i}]$ then there is some $m_i\in [0,1]$ for each $i\in[n]$ which
$$
\sv[f]\le \sum_{i=1}^n\delta_i^{m_i}(T)\shap_i[f]
$$
\end{theorem}

\begin{proof}
Define $m_i\in [0,1]$ to be a probability which maximizes $\delta_i^p(T)$. That is, $m_i=\argmax_{p\in [0,1]}\delta_i^p(T)$.
Combining the previous two lemmas we have
\begin{align*}
    \sv[f]&=\underset{p\sim[0,1]}{\E}\left[\Var_p[f]\right]\\
    &\le \underset{p\sim[0,1]}{\E}\left[\sum_{i=1}^n\delta_i^p(T)\Inf_{i,p}^{\hspace{0.1em}\text{OSSS}}[f]\right]\\
    &\le \underset{p\sim[0,1]}{\E}\left[\sum_{i=1}^n\delta_i^p(T)\Inf_{i,p}[f]\right]\\
    &=\sum_{i=1}^n\underset{p\sim[0,1]}{\E}\left[\delta_i^p(T)\Inf_{i,p}[f]\right]\\
    &\le \sum_{i=1}^n\delta_i^{m_i}(T)\underset{p\sim[0,1]}{\E}\left[\Inf_{i,p}[f]\right]\\
    &= \sum_{i=1}^n\delta_i^{m_i}(T)\shap_i[f].
\end{align*}
\end{proof}


This theorem is particularly useful since we can use it to prove that $\sv[f]\le 2d^2\max_i\shap_i[f]$ where $d$ is the depth of $T$. To do so, we first prove a lemma.

\begin{lemma}
\label{lem:delta_upper}
Let $T$ and $\delta_i^p(T)$ be as in the statement of Theorem \ref{theorem:osss} and let $m_i$ be as in the proof, then
$$
\sum_{i=1}^n\delta_i^{m_i}(T)\le d^2.
$$
\end{lemma}

\begin{proof}
We start by observing that it is sufficient to prove the statement in the case when $T$ is a read-once decision tree, that is, when each variable appears once in the tree. This follows from the observation that
\begin{align*}
    \underset{p\in [0,1]}{\max}\delta_i^p(T)&=\underset{p\in [0,1]}{\max}\Pr_p[T\text{ queries }x_i]\\
    &=\underset{p\in [0,1]}{\max}\sum_{\substack{v\in T\\{v=x_i}}}\Pr_p[T\text{ queries vertex } v]\\
    &\le \sum_{\substack{v\in T\\{v=x_i}}}\underset{p\in [0,1]}{\max}\Pr_p[T\text{ queries vertex } v].
\end{align*}

For a vertex $v\in T$ occurring at depth $k$, let $x_v\in\{0,1\}^k$ be the string representing the path from the root to $v$. Hence $\Pr_p[T\text{ queries vertex } v]=p^{|x_v|}(1-p)^{k-|x_v|}$ where $|x_v|$ is the \textit{Hamming weight} of $x_v$. The maximum of $p^{|x_v|}(1-p)^{k-|x_v|}$ over $p$ occurs at $p*=|x_v|/k$ and the maximum probability at this value is $(|x_v|/k)^{|x_v|}(1-|x_v|/k)^{k-|x_v|}$. Note that the maximum only depends on the depth of $v$ and the Hamming weight of $|x_v|$. Hence, for a given $v$, there will be $\binom{k}{|x_v|}$ total vertices at depth $k$ with the same maximum probability. We can then write
\begin{align*}
    \sum_{\substack{v\in T\\v\text{ at depth }k}}\underset{p\in [0,1]}{\max}\Pr_p[T\text{ queries vertex } v]&=\sum_{i=0}^k\binom{k}{i}\paren{\frac{i}{k}}^i\paren{1-\frac{i}{k}}^{k-i}\\
    &\le k+1
\end{align*}
where the last step follows from bounding each term in the sum by $1$. Specifically, we can note that 
$$
\Pr[X=i]=\binom{k}{i}\paren{\frac{i}{k}}^i\paren{1-\frac{i}{k}}^{k-i}\le 1
$$
where $X$ is a binomially distributed random variable over $k$ experiments each with probability $i/k$ of success. It follows that
\begin{align*}
    \sum_{i=1}^n\delta_i^{m_i}(T)&\le \sum_{k=1}^d\sum_{\substack{v\in T\\v\text{ at depth }k}}\underset{p\in [0,1]}{\max}\Pr_p[T\text{ queries vertex } v]\\
    &\le \sum_{k=1}^d k+1\\
    &\le d^2.
\end{align*}
\end{proof}

\begin{corollary}
Let $f$ be a Boolean function computed by a depth $d$ decision $T$, then
$$
\sv[f]\le 2d^2\max_i\shap_i[f].
$$
\end{corollary}
\begin{proof}
Combining Lemma \ref{lem:delta_upper} and Theorem \ref{theorem:osss} we write
\begin{align*}
    \sv[f]&\le 2\sum_{i=1}^n\delta_i^{m_i}(T)\shap_i[f]\\
    &\le 2\max_i\shap_i[f]\sum_{i=1}^n\delta_i^{m_i}(T)\\
    &\le  2d^2\max_i\shap_i[f].
\end{align*}
\end{proof}

The Theorems \ref{theorem:osss} and \ref{theorem:sv_lower} culminate in the following lower bound on the maximum Shapley value of a function $f$.

\begin{corollary}
Let $f$ be a nonconstant, monotone function computed by a depth $d$ decision tree. Then,
$$
\max_i\shap_i[f]\ge \Omega\paren{\frac{1}{d^3}}.
$$
\end{corollary}

\begin{proof}
Theorems \ref{theorem:osss} and \ref{theorem:sv_lower} show that
$$
2d^2\max_i\shap_i[f]\ge\sv[f]\ge \Omega\paren{\frac{1}{d}}
$$
which in turns shows
$$
\max_i\shap_i[f]\ge \Omega\paren{\frac{1}{d^3}}.
$$
\end{proof}

